Interfacing Automatic Proof Agents in Atelier B: Introducing "iapa"

The application of automatic theorem provers to discharge proof obligations is necessary to apply formal methods in an efficient manner. Tools supporting formal methods, such as Atelier~B, generate proof obligations fully automatically. Consequently, such proof obligations are often cluttered with information that is irrelevant to establish their validity. We present iapa, an "Interface to Automatic Proof Agents", a new tool that is being integrated to Atelier~B, through which the user will access proof obligations, apply operations to simplify these proof obligations, and then dispatch the resulting, simplified, proof obligations to a portfolio of automatic theorem provers.

==> abstract.tex <==
\begin{abstract}
The application of automatic theorem provers to discharge proof obligations
is necessary to apply formal methods in an efficient manner. Tools supporting
formal methods, such as Atelier~B, generate proof obligations fully automatically.
Consequently, such proof obligations are often cluttered with information that is
irrelevant to establish their validity. 

We present iapa, an ``Interface to Automatic Proof Agents'', a new tool that is
being integrated to Atelier~B, through which the user will access proof 
obligations, apply operations to simplify these proof obligations, and then
dispatch the resulting, simplified, proof obligations to a portfolio of 
automatic theorem provers.
\end{abstract}


==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{C. Dubois, P. Masci, D. M\'ery (Eds.): F-IDE 2016\\
EPTCS 240, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.240.6}{10.4204/EPTCS.240.6}}
\pdfoutput=1

